Towards a Mechanistic Interpretation of Multi-Step Reasoning Capabilities of Language Models

Recent work has shown that language models (LMs) have strong multi-step (i.e., procedural) reasoning capabilities. However, it is unclear whether LMs perform these tasks by cheating with answers memorized from pretraining corpus, or, via a multi-step reasoning mechanism. In this paper, we try to answer this question by exploring a mechanistic interpretation of LMs for multi-step reasoning tasks. Concretely, we hypothesize that the LM implicitly embeds a reasoning tree resembling the correct reasoning process within it. We test this hypothesis by introducing a new probing approach (called MechanisticProbe) that recovers the reasoning tree from the model's attention patterns. We use our probe to analyze two LMs: GPT-2 on a synthetic task (k-th smallest element), and LLaMA on two simple language-based reasoning tasks (ProofWriter & AI2 Reasoning Challenge). We show that MechanisticProbe is able to detect the information of the reasoning tree from the model's attentions for most examples, suggesting that the LM indeed is going through a process of multi-step reasoning within its architecture in many cases.

==> main_text/proposal.tex <==
\begin{abstract}
% background
Reasoning is a complex NLP task that requires various knowledge for solving it. Existing pretrained language models (LMs) have been more and more powerful, where rich factual knowledge, commonsense knowledge, etc., are learned from massive corpus with big model capacity.
% challenge
However, reasoning is always done in a procedural manner. Except aforementioned descriptive knowledge, procedural knowledge is also required, which is more abstract and contains rich explicit and implicit rules. 
%% introduce generalization
Simply using overparameterized LMs to fit inductive biases generally comes at the cost of decreasing the universality of LM~\citep{lmgeneralization_deletang22}, which is vital for models to learn and generalize rules. Overfitting these biases can work well for descriptive knowledge but not for procedures. 

% what we can do
Therefore, in this project, we can explore the generalization abilities of LMs for some special domains of reasoning.
The general idea is to show that (large) LMs do reasoning based on the large corpus instead of powerful generalization ability. Thus, for some strong rule-based tasks such as arithmetic operations (subtraction, summation), they can only generalize across commonly seen data (e.g., short digit numbers).
There are three points to solve the rule-based tasks:
\begin{itemize}
    \item 1. Analysis. We can design some reasoning tasks which requires (large) LMs to extract rules. Then, we show that LMs cannot learn the rules, and the generalization mainly happens for similar data in the training set.
    \item 2. Enhance LMs with rules. We can categorize some important rules, and design special enhancement method to let LMs capture them. Then, we show with the enhancement, LMs can better generalize/perform with reasoning tasks (requiring those rules).
    \item 3. Reasoning with enhanced LMs in a compositional way. We can use modules (e.g., adapters), to enhance LMs with different rules as mentioned in point 2. Then, we design a ``parsing model'' to parse the question into multiple steps (e.g., reasoning trace) and solve this question with the set of enhanced modules (rule-based LMs).
\end{itemize}
\end{abstract}


\section{Motivation}
Even if LLMs such as GPT-3 perform well across different reasoning tasks, existing works have shown that (Large) LMs have some limitations about the generalization. \citet{recursionofthought_iclr23r} discusses that for the simple math calculation problem, LLMs can only perform well for short digits, which are commonly seen in the pretraining corpus. While for the long digits calculation, LLMs cannot solve it well.
However, using small models such as tiny Transformers and LSTMs (with carefully training and usage) can better extract these rules, and can achieve much better performance on the long digit math calculation.
Another example can be found in~\citep{rulebasednn_seo21}, it is difficult to use data-driven neural networks (i.e., supervised learning) to learn the rules of physical movements. 

This finding can be explained by model generalization. \citet{lmgeneralization_deletang22} mentioned that there is a tradeoff between fitting the inductive biases of natural language and model universality (i.e., generalizability). It implies that LLMs overfit much descriptive knowledge to achieve better performance for various NLP tasks, but at the same time, they lose the generalization ability to capture rules. And being able to learn these rules are important to many reasoning tasks.
%
Therefore, we can focus on some strong rule-based reasoning tasks, and improve their model generalizability to solve these tasks. 


\section{Reasoning Task Design}
There are many reasoning tasks that require models to learn the rules. From the empirical side, we can gather and categorize some well known reasoning datasets such as symbolic reasoning task (last letter prediction). But this is not that convincing and could bring some unnecessary workload.

Alternatively, I think we can follow the categorization of~\citet{lmgeneralization_deletang22}. In their Appendix 3, they propose a set of tasks (like some subtasks of symbolic reasoning and arithmetic reasoning) based on the Chomsky hierarchy. However, these samples are not natural sentences. We can follow their setting to gather / preprocess existing suitable datasets with similar task design, or we can generate them by our own (since we know and we can program these rules). 

Therefore, I formalize some rule-based reasoning tasks as follows. Note that this is the first draft version, and a better and more convincing categorization (based on other principle) may be proposed.

\paragraph{Grammar type: Regular.}
In this case, the reasoning order should be left-to-right. And there is no external memory to solve the task.
\begin{itemize}
    \item \textbf{1. Math}: 1-step operation; sequential operations (no order of  operations, e.g., parentheses)

    \textbf{Relevant dataset (subset)}: \href{https://aclanthology.org/N19-1246.pdf}{DROP}, 
    \href{https://aclanthology.org/2022.naacl-main.119.pdf}{OPERA},
    \href{https://allenai.org/data/lila}{Lila},
    \href{https://github.com/kojima-takeshi188/zero_shot_cot/blob/main/dataset/AddSub/AddSub.json}{AddSub dataset},
    \href{https://github.com/kojima-takeshi188/zero_shot_cot/blob/main/dataset/SVAMP/SVAMP.json}{SVAMP dataset}, 
    \href{https://www.deepmind.com/open-source/aqua-rat}{AQuA}, \href{https://openreview.net/pdf?id=H1gR5iR5FX}{DeepMind math dataset},
    \href{https://openreview.net/pdf?id=Pzj6fzU6wkj}{IsarStep}
    
    \item \textbf{2. State}: sequential state modeling (without using external memory)
    
    \textbf{Relevant dataset (subset)}: 
    \href{https://github.com/kojima-takeshi188/zero_shot_cot/blob/main/dataset/coin_flip/coin_flip.json}{Coin Flip dataset}, 
    \href{https://github.com/kojima-takeshi188/zero_shot_cot/blob/main/dataset/Bigbench_object_tracking/task.json}{Bigbench object tracking}.
\end{itemize}



\paragraph{Grammar type: Deterministic context-free.}
In this case, the reasoning order does not need to be sequential (left-to-right). It can be more complex using external memory, but the external memory functions as \textbf{stack}. 

\begin{itemize}
    \item \textbf{1. Math}: sequential operations with order manipulated by a stack, such as parenthesis
    \item \textbf{2. Reversing order}: print procedural with reverse order \href{https://transacl.org/ojs/index.php/tacl/article/viewFile/1325/299}{WikiHop}
    \item \textbf{3. Tree traversal}: subtask (e.g., traversal) of \href{https://allenai.org/data/entailmentbank}{EntailmentBank}
\end{itemize}

\paragraph{Grammar type: Context-sensitive.}
In this case, the reasoning order does not need to be sequential (left-to-right). It can be more complex using external memory that functions as \textbf{tape}. Note that even if theoretically the tape length should be finite, in practice we can regard it as infinite. 

\begin{itemize}
    \item \textbf{1. Math}: complex math equation solving problem
    \item \textbf{2. Repeat}: output the input sentence for multiple times. 
    \item \textbf{3. Sort}: NLI task/logical task/procedural text, sorting the order of them \href{https://transacl.org/ojs/index.php/tacl/article/viewFile/1325/299}{WikiHop}
\end{itemize}



\section{Potential Directions to Go}
\paragraph{Project 0: Benchmarks.} As mentioned in the abstract, we can first analyze existing LMs (as well as LLMs) on these tasks. We can show how they perform now similar to~\citet{lmgeneralization_deletang22} but in the reasoning scenario with natural sentences. Besides, we can also design some experiments to test their in-distribution and out-of-distribution performance. For example, the \href{https://allenai.org/data/lila}{Lila} dataset provides split data with two settings. We can also construct something similar by ourselves.

\iffalse
\textbf{Direction 1.} 
We can follow~\citet{lmgeneralization_deletang22}, and explore some interesting modules such as external memory modules to enhance LMs generalizability. 
\textbf{Pros.} This direction explore more essential drawbacks of Transformer-based models. The findings could be inspiring for researchers who are interested in using LMs to solve specific problems. For example, perhaps LMs cannot know how to solve math reasoning problems because of the architecture design (even though they are theoretically Turing complete).
\textbf{Cons.} This direction is quite challenging. First, it's hard to know the hypothesis set of LMs, and LMs are pretrained with different engineering tricks. It's extremely hard to develop an enhancement module from the theoretical side. Even if we can do that, it's may not work in practice.
\fi

\paragraph{Project 1 \& 2.} We can follow our previous work about knowledge enhancement for LMs. The focus here is to develop LMs to solve reasoning tasks.

\textbf{1}. We can focus on enhancing LM, exploring how to enhance the LM with small modules with better generalizability / performance. 

We can design a system to do the rule-based reasoning tasks. Using some new modules (e.g., adapters) and referring to~\citet{rulebasednn_seo21} to enhance LMs with rules. 

\textbf{2}. We can focus on the ``Parsing LM'', analyzing how to parse the question, and decompose it into multiple steps with correct order. 

There is one ``Parsing LM'' that can decompose questions into different steps (e.g., parsing complex math equations). Another LM with a set of ``adapters'' (could be prefix or other modules) is used to do one-step reasoning/operation. Based on the rules (e.g., subtraction, summation operations), corresponding modules can be selected and used to calculate the operation.

\textbf{3*}. Besides, we can focus on the interpretability. For example, we can use simple adapters for the enhancement, but design a model to learn how to compose them to solve the task. The model could be the ``Parsing LM'' or other simple learning method (e.g., gated fusion mechanism). The composition can reveal some insights about how LMs do the sequential reasoning inside it.



\iffalse
% preparation
Give a set of training data as supervised signals $D_{S} = \{ (\vx_1, \vy_1), (\vx_2, \vy_2), ... \}$, which are sampled from distribution $\mathbb{P}_{S}$. The test data $D_{T} = \{ (\vx_1, \vy_1), (\vx_2, \vy_2), ... \}$ are sampled from distribution $\mathbb{P}_{T}$. Here, $\vx_i$ is the input text (e.g., questions), and $\vy_i$ is the output text (e.g., answers). Note that here $\mathbb{P}_{S}$ and $\mathbb{P}_{T}$ could not be the same, i.e., test samples could be out-of-distribution. The problem here is to select samples from $D_{S}$ as the set $D_{S}' \subseteq D_{S}$ for in-context learning such that the generalization error is as small as possible.

% prove that a proper D_{S}' could cover the gap between P_S and P_T
We first show that the empirical risk of $D_{S}'$ is equivalent to the risk on test samples under a proper sampling strategy.
\begin{proposition}[Optimal Existence~\citep{DBLP:conf/alt/CortesMRR08}]
    Let the weight of sampling on $\vx_i$ is $w(\vx_i) = {\mathbb{P}_{T}(\vx_i, \vy_i)}/{\mathbb{P}_{S}(\vx_i, \vy_i)}$. Given a hypothesis $h\in \mathcal{H}$ and a cost of error function on it as $\rho_{h}(\cdot, \cdot)$, we have the risk on test set as
    \begin{equation}
        R_T(h) = \mathbb{E}_{D_{T} \sim \mathbb{P}_{T}}[\widehat{R}_{D_{T}}(h)] \cong \mathbb{E}_{(\vx,\vy) \in D_{S}'}[\rho_{h}(\vx, \vy)].
    \end{equation}
\end{proposition}
\begin{proof}
    Since these samples are independent, we have
    \begin{align} 
        \mathbb{E}_{D_{T} \sim \mathbb{P}_{T}} & [\widehat{R}_{D_{T}}(h)] = \frac{1}{|D_{T}|} \sum_{(\vx, \vy) \in D_{T}} \mathbb{E}_{D_{T} \sim \mathbb{P}_{T}}[\rho_{h}(\vx, \vy)] \nonumber\\ 
        & = \mathbb{E}_{(\vx, \vy) \sim \mathbb{P}_{T}}[\rho_{h}(\vx, \vy)] \nonumber\\
        & = \mathbb{E}_{(\vx, \vy) \sim \mathbb{P}_{T}}[w(\vx) \frac{\mathbb{P}_{S}(\vx, \vy)}{\mathbb{P}_{T}(\vx, \vy)}\rho_{h}(\vx, \vy)] \nonumber\\
        & = \mathbb{E}_{(\vx, \vy) \sim \mathbb{P}_{S}}[w(\vx)\rho_{h}(\vx, \vy)] \nonumber\\
        & \cong \mathbb{E}_{(\vx, \vy) \in D_{S}}[w(\vx)\rho_{h}(\vx, \vy)] \nonumber\\
        & = \mathbb{E}_{(\vx, \vy) \in D_{S}'}[\rho_{h}(\vx, \vy)]. \nonumber
    \end{align}
\end{proof}
This proposition indicates that a proper sampling strategy can compensate the gap between $\mathbb{P}_{S}$ and $\mathbb{P}_{T}$. With the optimal strategy, minimizing the empirical risk on the sampled set $D_{S}'$ can reduce the risk on the test set. 
However, the optimal weights are unknown. Next, we discuss how to find a near-optimal $D_{S}'$.

% knowledge space: connect feature and label
\paragraph{Knowledge space.} Note that given a task, not all information in the input text $\vx$ is useful. Thus, we introduce the concept of knowledge space. Given a sample pair $(\vx, \vy)$, the hidden representation of $\vx$ in the knowledge space is denoted by $\vz$, which only includes useful knowledge in terms of $\vy$.

% smoothness assumption
\begin{assumption}[{Smoothness}] \label{as_sm}
    We assume that the hidden representation $\vz$ is smooth in terms of the label $\vy$. This leads to the $L_C$-Lipschitz continuity: given two input samples $\vx_i$, $\vx_j$, and their labels $\vy_i$, $\vy_j$, their hidden representations $\vz_i$, $\vz_j$ satisfy that
    \begin{equation}
        d(\vy_i, \vy_j) \leq L_C \cdot d(\vz_i, \vz_j),
    \end{equation}
where $L_C$ is the Lipschitz constant and $d(\cdot, \cdot)$ is the $L^{p}$-norm distance measurement ($p\geq 1$), i.e., 
\end{assumption} 
This assumption promises that questions with similar answers should be embedded closer in the knowledge space. In other words, the representation $\vz$ contains not only explicit knowledge such as facts, but also has implicit knowledge such as reasoning patterns.
Next, we give the upper bound of risk on test data, and show that the bound can be reduced by a properly sampled set $D_{S}'$.

% modeling test data risk
\begin{definition}[{Risk}] \label{def_risk}
    Given a hypothesis $h$ from the hypothesis class $\mathcal{H}$, the sampled training data $D_{S}'$ should minimize the risk on the distribution of test set as
    \begin{equation}
        R_T(h) \cong \widehat{R}_{D_{T}}(h) = \mathbb{E}_{(\vz, \vy) \in {D}_{T}}[d(h(\vz), \vy)].
    \end{equation}
\end{definition} 

\begin{definition}[{Dataset Smoothness}] \label{def_datasmooth}
    Similar to the Lipschitz continuity, we define the smoothness on dataset $D_{S}'$ as
    \begin{equation}
        \hat{L}_{D_{S}'} = \max_{(\vz, \vy), (\vz', \vy') \in D_{S}' } \left\{ \frac{d(\vy,\vy')}{d(\vz, \vz')} \right\}.
    \end{equation}
\end{definition} 

\begin{definition}[{Hypothesis Smoothness}] \label{def_hsmooth}
    Suppose the hypothesis $h\in \mathcal{H}$ can predict labels with some noise, i.e., 
    \begin{equation}
        h(\vz) = \vy + \sigma,
    \end{equation}
    where $\sigma$ is a random noise. Without loss of generality, we let $\mathbb{E}[\sigma] = 0$. Then, we can get the smoothness bound on $h$ as 
    \begin{equation}
        d(h(\vz), h(\vz')) \leq L_C [d(\vz, \vz') + 2\sigma] .
    \end{equation}
\end{definition} 

\begin{theorem}[{Risk Upper Bound}] \label{th_bound}
    Given a set of training data $D_{S}'$, the risk on test data can be bounded as
    \begin{align}
        \widehat{R}_{D_{T}}(h) & = \mathbb{E}_{(\vz, \vy) \in D_{T} } [d(h(\vz), \vy)]  \nonumber\\ 
        & \leq  2 L_C \cdot d(D_{S}', D_{T}) + 2 \hat{L}_{D_{S}'} \cdot d(D_{S}') \nonumber\\
        & \quad + \widehat{R}_{D_{S}'}(h) + \lambda \nonumber .
    \end{align}
    Here, $d(D_{S}', D_{T})$ is the minimum distance between test sample from $D_{T}$ and the training sample $\vz_m$ from $D_{S}'$ as
    \begin{equation}
        d(D_{S}', D_{T}) = \mathbb{E}_{(\vz, \vy) \in D_{T} }[d(\vz, \vz_m)].
    \end{equation}
    And $d(D_{S}')$ is the minimum distance between $\vz_m$ and all training samples from $D_{S}'$ as
    \begin{equation}
        d(D_{S}') = \mathbb{E}_{(\vz', \vy') \in D_{S}'}\left[d(\vz' , \vz_m)\right].
    \end{equation}
    $\widehat{R}_{D_{S}'}(h)$ is the empirical risk on $D_{S}'$ and $\lambda$ here is a noise factor as 
    \begin{equation}
        \lambda = 2(L_C+\hat{L}_{D_{S}'})||\sigma|| .
    \end{equation}
\end{theorem} 
\begin{proof}
    The idea of this proof can be found in Figure~\ref{fig:proof_idea}.
    \begin{figure}[!htbp]
    	\centering
    	\includegraphics[width=1.\linewidth]{./figures/prove_sketch.png}
    	\vspace{-.2cm}
    	\caption{The risk on test sample can be divided by two main terms. }
    	\vspace{-.2cm}
    	\label{fig:proof_idea}
    \end{figure}
    We consider the risk bound with one test sample $(\vx, \vy)$, where the corresponding representation in knowledge space is $\vz$. Since the distance measurement is $p$-norm with $p\geq 1$, we have that the measurement is convex with Minkowski inequality~\citep{minkowski1910geometrie}. 
    Then, based on its triangle inequality and convexity, we have
    \begin{align}
        d(h(\vz), \vy) &  \leq  d(h(\vz) , \mathbb{E}_{(\vz', \vy') \in D_{S}'}[h(\vz')])  \nonumber\\
        &  \quad + d(\mathbb{E}_{(\vz', \vy') \in D_{S}'}[h(\vz')], \mathbb{E}_{(\vz', \vy') \in D_{S}'}[\vy'])  \nonumber\\
        &  \quad + d(\mathbb{E}_{(\vz', \vy') \in D_{S}'}[\vy'], \vy) \nonumber\\
        & \leq  \mathbb{E}_{(\vz', \vy') \in D_{S}'}\left[d(h(\vz) , h(\vz'))\right]  \nonumber\\
        & \quad + \mathbb{E}_{(\vz', \vy') \in D_{S}'}\left[d(h(\vz'), \vy')\right]  \nonumber\\
        & \quad + \mathbb{E}_{(\vz', \vy') \in D_{S}'}\left[d(\vy', \vy)\right]. \nonumber
    \end{align}
    The \textbf{second term} is the empirical risk on $D_{S}'$ as 
    \begin{equation}
        \widehat{R}_{D_{S}'}(h) = \mathbb{E}_{(\vz', \vy') \in D_{S}'}\left[d(h(\vz'), \vy')\right]. \nonumber
    \end{equation}
    Let $\vz_{m}$ denote the sample in $D_{S}'$ with closest distance to $\vz$, i.e., we have 
    \begin{equation} \nonumber
        d(\vz, \vz_{m}) = \min_{\vz' \in D_{S}'} {d(\vz, \vz')}.
    \end{equation}
    The \textbf{first term} can be bounded as below. Since we have
    \begin{align}
        d(h(\vz) , h(\vz')) & \leq d(h(\vz) , h(\vz_m)) + d(h(\vz_m) , h(\vz')) \nonumber\\
        & \leq L_C \left[d(\vz, \vz_m) + 2||\sigma||\right] \nonumber\\
        & \quad + \hat{L}_{D_{S}'} \left[d(\vz', \vz_m) + 2||\sigma||\right]  \nonumber, 
    \end{align}
    we can then get that 
    \begin{align}
        \mathbb{E}_{(\vz', \vy') \in D_{S}'}&\left[d(h(\vz) , h(\vz'))\right] \leq  L_C \cdot d(\vz, \vz_m)  \nonumber\\
        & \quad  + \hat{L}_{D_{S}'} \mathbb{E}_{(\vz', \vy') \in D_{S}'}\left[d(\vz' , \vz_m)\right]  \nonumber \\
        & \quad + 2(L_C+\hat{L}_{D_{S}'})||\sigma||. \nonumber
    \end{align}
    Similarly, we can bound the \textbf{third term} as
    \begin{align}
        \mathbb{E}_{(\vz', \vy') \in D_{S}'}&\left[d(\vy', \vy)\right] \leq L_C \cdot d(\vz, \vz_m) \nonumber\\
        & \quad + \hat{L}_{D_{S}'} \mathbb{E}_{(\vz', \vy') \in D_{S}'}\left[d(\vz' , \vz_m)\right]  \nonumber
    \end{align}
    Therefore, we can get the bound for $d(h(\vz), \vy)$ as 
    \begin{align}
        d(h(\vz), \vy) & \leq \widehat{R}_{D_{S}'}(h) + 2 L_C \cdot d(\vz, \vz_m) \nonumber\\
        & \quad + 2 \hat{L}_{D_{S}'} \mathbb{E}_{(\vz', \vy') \in D_{S}'}\left[d(\vz' , \vz_m)\right] \nonumber\\
        & \quad + 2(L_C+\hat{L}_{D_{S}'})||\sigma||. \nonumber
    \end{align}
\end{proof}

\fi
